Tiered-Latency DRAM: Enabling Low-Latency Main Memory at Low Cost

This paper summarizes the idea of Tiered-Latency DRAM (TL-DRAM), which was published in HPCA 2013, and examines the work's significance and future potential. The capacity and cost-per-bit of DRAM have historically scaled to satisfy the needs of increasingly large and complex computer systems. However, DRAM latency has remained almost constant, making memory latency the performance bottleneck in today's systems. We observe that the high access latency is not intrinsic to DRAM, but a trade-off is made to decrease the cost per bit. To mitigate the high area overhead of DRAM sensing structures, commodity DRAMs connect many DRAM cells to each sense amplifier through a wire called a bitline. These bit-lines have a high parasitic capacitance due to their long length, and this bitline capacitance is the dominant source of DRAM latency. Specialized low-latency DRAMs use shorter bitlines with fewer cells, but have a higher cost-per-bit due to greater sense amplifier area overhead. To achieve both low latency and low cost per bit, we introduce Tiered-Latency DRAM (TL-DRAM). In TL-DRAM, each long bitline is split into two shorter segments by an isolation transistor, allowing one of the two segments to be accessed with the latency of a short-bitline DRAM without incurring a high cost per bit. We propose mechanisms that use the low-latency segment as a hardware-managed or software-managed cache. Our evaluations show that our proposed mechanisms improve both performance and energy efficiency for both single-core and multiprogrammed workloads. Tiered-Latency DRAM has inspired several other works on reducing DRAM latency with little to no architectural modification.

==> sty/mysty.tex <==
\usepackage[nocompress]{cite}
\usepackage{algorithmic}
\usepackage{array}

\makeatletter
\let\MYcaption\@makecaption
\makeatother

\usepackage[font=footnotesize]{subcaption}

\makeatletter
\let\@makecaption\MYcaption
\makeatother

\usepackage{fixltx2e}
\usepackage{dblfloatfix}
\usepackage[nolessnomore, italic]{mathastext}
\usepackage[T1]{fontenc}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage[normalem]{ulem}
\usepackage{enumitem}
\usepackage{setspace}
\usepackage{indentfirst}
\usepackage{footmisc}
\usepackage{fancyhdr}
\usepackage{authblk}
\usepackage[binary-units=true]{siunitx}
\usepackage[us,12hr]{datetime}
\usepackage[keeplastbox]{flushend}
\usepackage[hidelinks]{hyperref}

\usepackage{url}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stmaryrd}
\usepackage{indentfirst}
\usepackage{footnote}
\usepackage{float}
%\usepackage{subfig}
\usepackage{gensymb}
\newcommand{\mycolor}[1]{\textcolor{black}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}   %comment command for Onur
\newcommand{\checkit}[1]{\textcolor{red}{\textbf{#1}}}

\newcommand\numone{{\large \ding{192}}\xspace}
\newcommand\numtwo{{\large \ding{193}}\xspace}
\newcommand\numthree{{\large \ding{194}}\xspace}
\newcommand\numfour{{\large \ding{195}}\xspace}
\newcommand\numfive{{\large \ding{196}}\xspace}
\newcommand\trc{$t_{\mathit{RC}}$\xspace}
\newcommand\trcd{$t_{\mathit{RCD}}$\xspace}
\newcommand\tcl{$t_{\mathit{CL}}$\xspace}
\newcommand\tcwl{$t_{\mathit{CWL}}$\xspace}
\newcommand\tbl{$t_{\mathit{BL}}$\xspace}
\newcommand\tras{$t_{\mathit{RAS}}$\xspace}
\newcommand\trp{$t_{\mathit{RP}}$\xspace}
\newcommand\vdd{$V_{\mathit{DD}}$\xspace}
\newcommand\trcdfar{$t_{\mathit{RCDfar}}$\xspace}
\newcommand\trcfar{$t_{\mathit{RCfar}}$\xspace}
\newcommand\trcdnear{$t_{\mathit{RCDnear}}$\xspace}
\newcommand\trcnear{$t_{\mathit{RCnear}}$\xspace}
\newcommand\trasnear{$t_{\mathit{RASnear}}$\xspace}
\newcommand\trasfar{$t_{\mathit{RASfar}}$\xspace}
\newcommand\trpnear{$t_{\mathit{RPnear}}$\xspace}
\newcommand\trpfar{$t_{\mathit{RPfar}}$\xspace}
\newcommand\cmdact{ACTIVATE\xspace}
\newcommand\cmdpre{PRECHARGE\xspace}
\newcommand\cmdrd{READ\xspace}
\newcommand\cmdwr{WRITE\xspace}
\newcommand\ra{$\rightarrow$}
\newcommand{\msc}{SC\xspace}
\newcommand{\mtac}{WMC\xspace}
\newcommand{\mbbc}{BBC\xspace}
\newcommand{\trccritical}{\trc-\emph{critical}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compactify for floats
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\floatsep}{10pt}
\setlength{\dblfloatsep}{10pt}
\setlength{\textfloatsep}{5pt}
\setlength{\dbltextfloatsep}{5pt}
\setlength{\intextsep}{5pt}
\addtolength{\abovecaptionskip}{-5pt}
%\setlength{\belowcaptionskip}{-1pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compactify for text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{setspace}
%\usepackage{sty/bibspacing}
% \setlength{\columnsep}{0.18in}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% prevent footnotes from crossing pages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\interfootnotelinepenalty=10000
%\widowpenalty=10000
%\clubpenalty=10000
% \pagestyle{plain}


